Monte Carlo Information-Oriented Planning

In this article, we discuss how to solve information-gathering problems expressed as rho-POMDPs, an extension of Partially Observable Markov Decision Processes (POMDPs) whose reward rho depends on the belief state. Point-based approaches used for solving POMDPs have been extended to solving rho-POMDPs as belief MDPs when its reward rho is convex in B or when it is Lipschitz-continuous. In the present paper, we build on the POMCP algorithm to propose a Monte Carlo Tree Search for rho-POMDPs, aiming for an efficient on-line planner which can be used for any rho function. Adaptations are required due to the belief-dependent rewards to (i) propagate more than one state at a time, and (ii) prevent biases in value estimates. An asymptotic convergence proof to epsilon-optimal values is given when rho is continuous. Experiments are conducted to analyze the algorithms at hand and show that they outperform myopic approaches.

==> Makefile <==
DEPS_DIR = .deps
LATEXMK = latexmk -recorder -use-make -deps \
	-e 'warn qq(In Makefile, turn off custom dependencies);' \
	-e '@cus_dep_list = ();' \
	-e 'show_cus_dep();'

ecai_2020.pdf : ecai_2020.tex Makefile
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	-$(LATEXMK) -pdf -deps-out=$(DEPS_DIR)/$@P $<
	./clean-deps.sh $(DEPS_DIR)/$@P

clean :
	rm -f *~
	latexmk -c

veryclean:
	rm -rf *~ .deps *.bbl figures/*.bak
	latexmk -C

